Integer superharmonic matrices on the $F$-lattice

We prove that the set of quadratic growths achievable by integer superharmonic functions on the $F$-lattice, a periodic subgraph of the square lattice with oriented edges, has the structure of an overlapping circle packing. The proof recursively constructs a distinct pair of recurrent functions for each rational point on a hyperbola. This proves a conjecture of Smart (2013) and completely describes the scaling limit of the Abelian sandpile on the $F$-lattice.

==> Figures/tiles/README <==
figures are generated by
/home/nitro/Desktop/F_Lattice/construct_odometer/annotated_tiles/gen_figs.jl

they represent all the possible tile orientations and overlaps 
in both the standard case and the alternate case 

even-first orientation e_*
odd-first o_*

even tile _*q, odd tile _*q

type i\in{1,2,3} child *i*

the notation for the subtiles is as the written document

